AU-TTT: Vision Test-Time Training model for Facial Action Unit Detection

Facial Action Units (AUs) detection is a cornerstone of objective facial expression analysis and a critical focus in affective computing. Despite its importance, AU detection faces significant challenges, such as the high cost of AU annotation and the limited availability of datasets. These constraints often lead to overfitting in existing methods, resulting in substantial performance degradation when applied across diverse datasets. Addressing these issues is essential for improving the reliability and generalizability of AU detection methods. Moreover, many current approaches leverage Transformers for their effectiveness in long-context modeling, but they are hindered by the quadratic complexity of self-attention. Recently, Test-Time Training (TTT) layers have emerged as a promising solution for long-sequence modeling. Additionally, TTT applies self-supervised learning for iterative updates during both training and inference, offering a potential pathway to mitigate the generalization challenges inherent in AU detection tasks. In this paper, we propose a novel vision backbone tailored for AU detection, incorporating bidirectional TTT blocks, named AU-TTT. Our approach introduces TTT Linear to the AU detection task and optimizes image scanning mechanisms for enhanced performance. Additionally, we design an AU-specific Region of Interest (RoI) scanning mechanism to capture fine-grained facial features critical for AU detection. Experimental results demonstrate that our method achieves competitive performance in both within-domain and cross-domain scenarios.

==> Equation/Loss.tex <==


\begin{equation}
\mathcal{L} = \lambda_{\text{MDWA}}\cdot\mathcal{L}_{\text{MDWA}} + \lambda_{\text{WDI}}\cdot\mathcal{L}_{\text{WDI}} + \lambda_{\text{MSE}}\cdot\mathcal{L}_{\text{MSE}},
\end{equation}

==> Equation/MDWAloss.tex <==
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{MDWA}} = -\frac{1}{N} \sum_{i=1}^N \omega_i & [ y_i \log(p_i) \\
& + (1 - y_i) p_{m,i}^{\gamma_i} \log(1 - p_{m,i}) ],
\end{aligned}
\label{equation:MDWAloss}
\end{equation}

==> Equation/MSEloss.tex <==

\begin{equation}
\mathcal{L}_{MSE} = \| m - \hat{m} \|_2^2,
\end{equation}

==> Equation/WDIloss.tex <==
\begin{equation}
\mathcal{L}_{\text{WDI}} = \frac{1}{N} \sum_{i=1}^{N} \omega_i \left(1 - \frac{2 y_i p_i + \epsilon}{y_i^2 + p_i^2 + \epsilon} \right),
\label{equation:WDIloss}
\end{equation}

==> Equation/bittt.tex <==
\begin{equation}
\begin{aligned}
\text{Bi-TTT}(\mathbf{Z}) 
&= \text{Bi-TTT}([\mathbf{z}^1; \mathbf{z}^2; \dots; \mathbf{z}^J; \text{CLS}]) \\
&= \text{Linear}(\text{Cat}(\text{TTT}([\mathbf{z}^1; \mathbf{z}^2; \dots; \mathbf{z}^J; \text{CLS}]) \\
&\qquad \text{Reverse}(\text{TTT}([\mathbf{z}^J; \mathbf{z}^{J-1}; \dots; \mathbf{z}^1; \text{CLS}])))).
\end{aligned}
\end{equation}

==> Figure/bittt.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figure/bi_ttt.pdf} % Replace with your file name
    \vspace{-2em}
    \caption{BiTTT.}
    \vspace{-1.5em}
    \label{fig:bittt} % For referencing the figure
\end{figure}

==> Figure/cross_gap.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figure/performance_gap.pdf} % Replace with your file name
    \caption{Performance (F1 score) gap between the within- and cross-domain AU detection for DRML, J$\hat{\mathrm{A}}$A-Net, MEGraphAU, FG-Net, AUFormer, and AU-TTT(Ours). The within-domain performance is averaged between DISFA and BP4D, while the cross-domain performance is averaged between BP4D to DISFA and DISFA to BP4D.}
    \label{fig:performance_gap} % For referencing the figure
\end{figure}

==> Figure/framework.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/framework_arc.pdf} % Replace with your file name
    \caption{\textbf{Top Left}: The overall AU-TTT framework. \textbf{Top Right}: The architecture of the AU-TTT Block. \textbf{Bottom Left}: The original TTT Layer scanning method. \textbf{Bottom Center}: The bidirectional TTT scanning method. \textbf{Bottom Right}: The AU RoI TTT scanning method.}
    \label{fig:framework} % For referencing the figure
\end{figure*}

==> Figure/tttlayer.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Figure/TTTlayer.pdf} % Replace with your file name
    \caption{\textbf{A}: Original TTT Block. \textbf{B}: Original TTT Layer. \textbf{C}: Hidden state update rule.}
    \label{fig:tttlayer} % For referencing the figure
\end{figure*}

==> Table/cross_domain.tex <==
\begin{table*}[t]
\caption{F1-scores (in \%) for cross-domain evaluations between BP4D and DISFA. The best and second best results for each column are bolded and underlined, respectively. $^*$The numbers are derived from a replication of \cite{yin2024fg} based on open-source code.
}
\centering

\begin{tabular}{l|ccccc|c|ccccc|c}
\toprule

Direction & \multicolumn{6}{c|}{BP4D $\rightarrow$ DISFA} & \multicolumn{6}{c}{DISFA $\rightarrow$ BP4D} \\
\midrule

AU & 1 & 2 & 4 & 6 & 12 & \textbf{Avg.} & 1 & 2 & 4 & 6 & 12 & \textbf{Avg.} \\
\midrule
DRML$^*$ \cite{zhao2016deep} & 10.4 & 7.0 & 16.9 & 14.4 & 22.0 & 14.1 & 19.4 & 16.9 & 22.4 & 58.0 & 64.5 & 36.3  \\
J{\^A}A-Net$^*$ \cite{shao2021jaa} & 12.5 & 13.2 & 27.6 & 19.2 & 46.7 & 23.8 & 10.9 & 6.7 & 42.4 & 52.9 & 68.3 & 36.2  \\
ME-GraphAU$^*$ \cite{luo2022learning} & 43.3 & 22.5 & 41.7 & 23.0 & 34.9 & 33.1 & 36.5 & 30.3 & 35.8 & 48.8 & 62.2 & 42.7  \\

Patch-MCD \cite{yin2021self} & 34.3 & 16.6 & \textbf{52.1} & 33.5 & 50.4 & 37.4 & - & - & - & - & - & -  \\
BG-AU~\cite{cui2023biomechanics} & - & - & - & - & - & 38.8 & - & - & - & - & - & -  \\
IdenNet \cite{tu2019idennet} & 20.1 & 25.5 & 37.3 & \textbf{49.6} & \textbf{66.1} & 39.7 & - & - & - & - & - & -  \\
FG-Net~\cite{yin2024fg}  & \textbf{61.3} & \textbf{70.5} & 36.3 & \underline{42.2} & \underline{61.5} & \textbf{54.4} & \textbf{51.4} & \textbf{46.0} & 36.0 & 49.6 & 61.8 & 49.0 \\
AUFormer~\cite{yuan2025auformer} & \underline{49.7} & \underline{49.9} & \underline{43.2} & 31.5 & 43.5 & \underline{43.6} & \underline{49.8} & \underline{43.8} & \textbf{45.7} & \underline{66.6} & \underline{74.5} & \underline{56.1}  \\
\midrule
\rowcolor{gray!30}
\textbf{AU-TTT (Ours)} &  &  &  &  &  &  & 49.0 & 39.1 & \underline{45.6} & \textbf{72.8} & \textbf{77.5} &  
\textbf{56.8} \\

\bottomrule
\end{tabular}
\label{tab:cross_domain}
\end{table*}

==> Table/within_domain.tex <==
\begin{table}[t] % Changed to [t] to specify table positioning at the top of the page
\centering
\caption{Average F1-score (in \%) results for within-domain evaluations on BP4D and DISFA. The best and second-best results for each column are bolded and underlined, respectively.}
\label{tab:DISFA_BP4D}

\begin{tabular}{l|c|cc}
\toprule
Method & Venue & BP4D & DISFA \\
\midrule
DRML~\cite{zhao2016deep} & CVPR 16 & 48.3 & 26.7 \\
LP-Net~\cite{niu2019local} & CVPR 19 & 61.0 & 56.9 \\
SRERL~\cite{li2019semantic} & AAAI 19 & 62.9 & 55.9 \\
J{\^A}A-Net~\cite{shao2021jaa} & IJCV 21 & 62.4 & 63.5 \\
HMP-PS~\cite{song2021hybrid} & CVPR 21 & 63.4 & 61.0 \\
SEV-Net~\cite{yang2021exploiting} & CVPR 21 & 63.9 & 58.8 \\
FAUDT~\cite{jacob2021facial} & CVPR 21 & 64.2 & 61.5 \\
PIAP~\cite{tang2021piap} & ICCV 21 & 64.1 & 63.8 \\
KDSRL~\cite{chang2022knowledge} & CVPR 22 & 64.5 & 64.5 \\
ME-GraphAU~\cite{luo2022learning} & IJCAI 22 & 65.5 & 62.4 \\ 
BG-AU~\cite{cui2023biomechanics} & CVPR 23 & 64.1 & 58.2 \\
KS~\cite{li2023knowledge} & ICCV 23 & 64.7 & 62.8 \\
FG-Net~\cite{yin2024fg} & WACV 24 & 64.3 & 65.4 \\ 
AUFormer~\cite{yuan2025auformer} & ECCV 2024 & \textbf{66.2} & \textbf{66.4} \\

\midrule

\rowcolor{gray!30}
\textbf{AU-TTT (Ours)} & - & \underline{65.6} & \textbf{66.4} \\

\bottomrule
\end{tabular}
\end{table}
